Active propulsion noise shaping for multi-rotor aircraft localization

Multi-rotor aerial autonomous vehicles (MAVs) primarily rely on vision for navigation purposes. However, visual localization and odometry techniques suffer from poor performance in low or direct sunlight, a limited field of view, and vulnerability to occlusions. Acoustic sensing can serve as a complementary or even alternative modality for vision in many situations, and it also has the added benefits of lower system cost and energy footprint, which is especially important for micro aircraft. This paper proposes actively controlling and shaping the aircraft propulsion noise generated by the rotors to benefit localization tasks, rather than considering it a harmful nuisance. We present a neural network architecture for selfnoise-based localization in a known environment. We show that training it simultaneously with learning time-varying rotor phase modulation achieves accurate and robust localization. The proposed methods are evaluated using a computationally affordable simulation of MAV rotor noise in 2D acoustic environments that is fitted to real recordings of rotor pressure fields.

==> sections/030_dataset.tex <==
\section{Dataset}\label{sec:dataset}
Current publicly available auditory datasets of MAV and single rotors are few, and
consist of flyover data only, making the recordings vulnerable to aircraft movements
and external environmental disturbances, such as wind \cite{strauss2018dregon}. Therefore, to model the self sound of a rotor in free-space we recorded a new dataset of a single spinning rotor in a semi-anechoic room. 
The recording setup included a motor with a rotor mounted on a tripod, that was
placed in the middle of the room. A microphone array of four RODE
NTG4 directional shotgun microphones was placed circularly around the rotor to
capture the sound. To measure the instantaneous shaft position of the rotor an
encoder was mounted on the motor, and its readings were synchronized with the
microphones’ recordings using an audio interface, Roland OCTA-CAPTURE, at a
sampling rate of 44.1[kHz]. 

The four microphones were placed in $\frac{\pi}{2}$ [rad] angular distances from each other, and at each experiment
their distance was changed from the rotor’s origin. The experiments consisted in
total eight distances: [0.53, 0.57, 0.63, 0.68, 0.73, 0.83, 0.93, 1.03][m].

An open-loop control system was used to control the motor speed. The hardware
included a BeagleBoard with an Electronic Speed Controller (ESC) 40[A]. In each
experiment, the motor was rotated in 10 incremental angular velocities, each one for
a sequence of 5[sec].  The rotor’s instantaneous shaft position was
measured as a feedback to the control system, reading the encoder’s measurements.

The encoder’s data included two channels: incremental channel and indicator at a
reference position. Combining these two channels deduce the instantaneous shaft
position and the angular velocity of the motor. The incremental channel was discretized to 1024 readings per revolution. However, this precision and the sampling
rate determined the Nyquist frequency which limits the rotor angular velocity to
21.53[Hz] maximum to get a clean encoder signal. This velocity is considered to be
a low angular velocity for MAVs. Therefore, we down-sampled the encoder’s incremental channel to 128 readings per revolution. A low-pass Butterworth filter was
also applied to the encoder’s incremental channel for denoising, and a sign clipping
to create a square-shaped signal.

We show in \ref{fm} how we used the combination of the recordings with the encoder readings in order to create a differentiable simulator of the self sound of the drone. In \ref{phase modulation optimization} we will show how the differentiability of our simulator played a crucial role in learning the phase modulation that we used to increase the performance of our localization system.

==> sections/robustness_tests/090_robustness_tests_intro.tex <==
\section{Robustness Experiments}\label{sec:robustness_experiments}
We conducted several tests to assess the sensitivity of the model to the presence of noise in the recording and to some modelling error in the geometry of the room in which the sound has been recorded.

==> sections/robustness_tests/091_robustness_tests_sensor_noise.tex <==
\paragraph*{Sensor noise}
The pressure field recorded by the microphones is expected to include some noise coming from a variety of sources, such as recording system noise, or noise within the medium through which sound traverses. In this section we test the sensitivity of the model to these uncertainties. We do so by adding white Gaussian noise of different bandwidths to the input sound. Specifically, we assessed the performance of the model by inducing the following SNR levels: $[5, 10, \dots, 75]$ [dB]. First, we perform robust training of our localization mode. Namely, we train the model by injecting white Gaussian noise whose induced SNR has been chosen uniformly random among $25 dB,30 dB, 35dB$. After training we test performance in terms of RMS loss under all noise levels. Results are depicted in figure \ref{fig:robustness_test_noise}.




==> sections/robustness_tests/092_robustness_tests_environment_modeling_errors.tex <==
\paragraph*{Environment modeling errors} We evaluated the sensitivity of the trained localization model to mismatched environment parameters between training and test time. The following parameters were perturbed in isolation: \emph{uniform scale} of the environment ranging from $50\%$ to $200\%$ in terms of area, area-preserving \emph{aspect ratio} perturbations of the originally square environment in the range $0.5--2$, area-preserving \emph{shear deformations} in the range of $0-45^\circ$, and \emph{acoustic reflection coefficient} perturbation in the range of $0.05--0.95$ with nominal $\gamma=0.5$. Localization accuracy in response to these perturbations in depicted in Fig. \ref{fig:robustness}. In general, we can conclude that the model can gracefully cope with over $20\%$ deviations of the nominal environment parameters.

\subsubsection{Ratio Robustness} Due to the fact that we have trained our model in a square shaped room, we assessed the sensitivity of the model to the ratio between the sides of the room. In particular, in this test we deformed our original squared room so that one side of the room has been scaled up by a certain factor and the other side of the room has been scaled down by the inverse of this factor, thus keeping the area of the room constant.


\subsubsection{Shear Deformation} In this experiment we test the sensitivity of the model to the angle between the sides. For this reason we applied a shear transformation in order to assess the response of the model to a room with acute angles.


\subsubsection{Uniform Deformation} In this experiment we  test the sensitivity of the model to the area of the room. For this reason we uniformly scaled our room in order to track the response of the model to rooms of different sizes.


\subsubsection{Acoustic reflection coefficient $\gamma$}
In this experiment we test the sensitivity of the model to the acoustic reflection coefficient $\gamma$. For this reason we assessed the performance of the model over rooms with a $\gamma$ that is different from the one seen in training.
